Privacy Vulnerabilities in Marginals-based Synthetic Data

When acting as a privacy-enhancing technology, synthetic data generation (SDG) aims to maintain a resemblance to the real data while excluding personally-identifiable information. Many SDG algorithms provide robust differential privacy (DP) guarantees to this end. However, we show that the strongest class of SDG algorithms--those that preserve \textit{marginal probabilities}, or similar statistics, from the underlying data--leak information about individuals that can be recovered more efficiently than previously understood. We demonstrate this by presenting a novel membership inference attack, MAMA-MIA, and evaluate it against three seminal DP SDG algorithms: MST, PrivBayes, and Private-GSD. MAMA-MIA leverages knowledge of which SDG algorithm was used, allowing it to learn information about the hidden data more accurately, and orders-of-magnitude faster, than other leading attacks. We use MAMA-MIA to lend insight into existing SDG vulnerabilities. Our approach went on to win the first SNAKE (SaNitization Algorithm under attacK ... $\varepsilon$) competition.

==> resubmission.tex <==

\begin{center}
    \textbf{Description of How Prior Reviews were Addressed}\\
    Prior version was submitted to ICML 2024 with Paper ID: 9444
\end{center}




We propose a novel membership inference attack, MAMA-MIA, that is computationally light-weight with leading accuracy. In the version that we submitted to ICML 2024 (Paper ID: 9444), the reviewers recognized the novelty of our attack but expressed concerns regarding the lack of comparisons with prior work, as well as the clarity of certain technical details and experimental setups. 

In the new version that we are submitting to SatML 2025, we have addressed the reviewers' concerns by strengthening the paper with extensive experiments, comparisons with relevant related work, adapting MAMA-MIA to an additional state-of-the-art synthetic data generator (SDG), and improved clarity. 

We sincerely appreciate the ICML reviewers' feedback, which is attached below. It was thoughtful, specific, and highly-valuable in helping us to improve the rigor of our investigation. We describe below how we addressed their concerns:


\vspace{0.7em}
\noindent
\textbf{Additional Experiments}
\begin{itemize}[itemsep=7pt]
    \item \textbf{Comparison to related work}: 
    
    Reviewers noted their expectation to see the works \cite{houssiau2022tapas}, \cite{stadler2022synthetic}, \cite{meeus2023achilles}, and \cite{guepin2023synthetic} referenced. In this updated version, we provide a much more detailed discussion on related works. Two of the aforementioned papers (i.e. \cite{meeus2023achilles}, \cite{guepin2023synthetic}) are not applicable to our work, and we explain why in the paper in section \ref{sec:related_mias}. As far as the other two, we have added to our results section a thorough empirical comparison with the leading attack from the TAPAS library \cite{houssiau2022tapas}, which is an enhancement of the Groundhog attack described in \cite{stadler2022synthetic}.
    
    \item \textbf{Attack on latest SDGs}: 
    
    Reviewers brought to our attention a novel SDG from 2023, Private-GSD \cite{liu2023generating}, that falls within the scope of our work. They also criticized the poor results we achieved on RAP \cite{aydore2021differentially}. We now adapt MAMA-MIA to Private-GSD with strong results, thoroughly investigating its performance using different datasets, different size configurations, and while comparing this adaptation to attacks from related works.

    \hspace{7.5pt} We also emphasize, and provide more evidence for, why our adaptation of MAMA-MIA to RAP is not flawed, but rather is a result of RAP's low-utility data generation, consistent with others' findings. This information is presented in the appendix section \ref{sec:RAP}.
    
    \item \textbf{Additional settings and metrics}: 
    
    One reviewer asked for performing our membership inference experiments in the setting where the training data does not overlap with the auxiliary, or reference data. We now include results for two datasets where the training data does not overlap with the auxiliary data, and we show that the results are nearly identical.
    
    \item \textbf{Justification and clarity on choices of experiments}: 
    
    In the previous version, a reviewer pointed out that using AUC as our success metric would be much more standard than the ``membership advantage'' metric we used. In the current version, we update all of our experiments to AUC. In addition, we still present results of a competition that used membership advantage to evaluate our model. We also refocus our experiments to single membership inference (``single MI'') attacks instead of set membership inference (``set MI''). Even though set MI was the objective in the competition that motivated our work, single MI is much more common in the literature. We still provide set MI results in the appendix.
    
    \hspace{7.5pt} Additionally, our use of $\varepsilon = 1,000$ in our investigation brought valid criticisms. We address these by first providing more sound justification for why we use this setting, namely to gain insight into the success rate of the MIAs on synthetic data that was generated with (almost) no differential privacy guarantees. Second, we revise the paper and experiments to focus on the setting where $\varepsilon = 10$, which is considered much more reasonable and is used by related works.

    \hspace{7.5pt} A reviewer pointed out that we compared our attack against DOMIAS \cite{van2023membership} using only one of its suggested modules, KDE, and not BNAF. Despite the substantial computational cost of BNAF, we rerun our experiments for this updated version of the paper to show that DOMIAS using BNAF is ineffective for all of our attack settings.


    
\end{itemize}


\vspace{0.7em}
\noindent
\textbf{Clarifications}
\begin{itemize}[itemsep=7pt]
    \item \textbf{Precision and formalism}: 
    
    It was pointed out in our previous version that the work lacked a formalized problem description, discussion of the threat model, as well as definitions of marginals and our ``focal-points''--a term we introduce. We update the preliminaries of this paper to more rigorously provide each of these components.
    
    \item \textbf{Attack on different categories of SDGs}: 
    
    It has been criticized that MAMA-MIA's applicability to only marginals-based synthetic data generators lacks novelty. To address this, we make a more earnest attempt at demonstrating MAMA-MIA's generalizability to \textit{any} marginals-based SDG, as well as those that rely on similar statistics, like conditionals or using projection. For example, PrivBayes uses conditionals instead of marginals, and MST is arguably a marginals-based algorithm that uses projection, and Private-GSD uses ``queries'', which are essentially marginals over one-hot encoded data. Since marginals-based SDGs have been shown to produce the highest quality synthetic data \cite{tao2021benchmarking,pereira2023assessment}, we argue that an attack designed to exploit them with relative ease is significant. 
    
    \hspace{7.5pt} Lastly, we clarify in the paper that our improvement in \textit{accuracy} over other leading attacks isn't our main novelty; in this version, we present additional findings that highlight that MAMA-MIA's primary contribution is that it is orders-of-magnitude more efficient than the leading attack.

    % \item \textbf{Discussion on results}:
\end{itemize}

